Self-assembly and entropic effects in pear-shaped colloid systems: II. Depletion attraction of pear-shaped particles in a hard sphere solvent

We consider depletion effects of a pear-shaped colloidal particle in a hard-sphere solvent, for two different model realisations of the pear-shaped colloidal particle. The two models are the pear hard Gaussian overlap (PHGO) particles and the hard pears of revolution (HPR). The motivation for this study is to provide a microscopic understanding for the substantially different mesoscopic self-assembly properties of these pear-shaped colloids, in dense suspensions, that have been reported in the first part of this series. This is done by determining the differing depletion attraction via MC simulations of PHGO and HPR particles in a pool of a hard spherical solvent and comparing them with excluded volume calculations of numerically obtained ideal configurations on the microscopic level. While the HPR model behaves as predicted by the analysis of excluded volumes, the PHGO model showcases a preference for splay between neighbouring particles, which can be attributed to the special non-additive characteristics of the PHGO contact function. Lastly, we propose a potentially experimentally realisable pear-shaped particle model, the non-additive hard pear of revolution (NAHPR) model, which is based on the HPR model but also features non-additive traits similar to those of PHGO particles to mimic their depletion behaviour.

==> images/chapter.tex <==
%\chapter{Depletion interactions between pear-shaped particles in a hard sphere fluid}
\chapter{Depletion interactions between pears in a hard sphere fluid}
\label{sec:Depletion}

\begin{chapquote}{Ilya Prigogine}
``Entropy is the price of structure.''
\end{chapquote}

\begin{chapabstract}
\small 
This chapter analyses depletion effects that enable further contrast between the two pear-shaped particle models -- the PHGO and HPR pear-shaped particles. After a brief introduction to depletion mechanisms and excluded volume computations for colloidal systems, we investigate the depletion attraction for both pear models. Furthermore, we compare the favourable two pear-shaped particle arrangements in terms of excluded volume, which are determined by MC simulations of PHGO and HPR particles in a pool of a hard spherical solvent, with the numerically obtained and, according to the B\'ezier-curv-curvee representation of the pear-shape, ideal configurations. While the HPR model behaves as expected from the analysis of excluded volumes, the PHGO model showcases a preference for splay between neighbouring particles which can be attributed to the non-additive characteristics of the PHGO contact function. Lastly, we propose a third pear-shaped particle model, the non-additive hard pear of revolution (NAHPR) model, which is based on the HPR model but also features non-additive traits to copy the depletion behaviour of the PHGO particles.
\end{chapabstract}\\

The previous chapter showed that minor discrepancies between contact profiles of the PHGO and the HPR particles lead to significant differences in the appearance of mesophases, most notably the presence of bilayer and gyroid phases in PHGO pears and their absence in the HPR model (see \chap{sec:PhaseDiamgrams}). However, until now only single-component configurations have been considered. The distinct mannerisms in the self-assembly of one-component systems is a clear indicator that the two pear-shaped particle models have to be distinguished. Nevertheless, the exact nature of the difference on a microscopical level and a specific reason why the phase diagrams differ for the two contact functions is not yet clear, and is the subject of this chapter.\\ 

In all liquid crystal phases, obtained both for the PHGO and the HPR particle model, the arrangement of each pear is highly affected by a multitude of next nearest neighbours. This elaborate interplay of particles coupled with the aspherical pear-shape, which features a significant degree of complexity, makes a more detailed analysis of the direct influence between adjacent particles impracticable. Hence, we reduce the complexity of our simulations in the following and shift our focus to systems which encapsulate the fundamental features of pure two particle interactions. In particular, we are interested in the specific depletion interactions of the pear-shaped particles. Within a sea of hard sphere particles acting as a solvent, depletion causes an effective attraction between two objects. Moreover, this can be seen as an initial step to add a second ``solvent'' component to the pure-pear liquid crystal phases in order to mimic lipid-water systems in \chap{sec:Mixtures}.\\ 

This chapter is structured as follows: We first discuss the physics of depletion phenomena and the historical background of depletion interactions in \sect{sec:EntropicForces}. Here, however, we focus mainly on the central physical concepts. For a more detailed description of depletion, we refer to \zit{LT2011}. Then in \sect{sec:ExclVolCalc} the optimal arrangement of pears in terms of their excluded volume is identified using numerical tools. Next (\sect{sec:MCDepletion}) we perform MC simulations of two large pear-shaped particles within a solution of smaller hard spheres; This is done for both the PHGO and HPR particle models to compare the computational results with the previous predictions of the ideal excluded volume, obtained by the numerical technique. These allow us to pinpoint the specific differences between the two models more efficiently and to make better assumptions why the PHGO particle favours the formation of bilayer phases like the bilayer smectic or gyroid phase in contrast to the HPR particle. Finally in \sect{sec:OutlookDepletion}, we will give a short outlook, how bilayer phases could possibly be stabilised in monodisperse systems based on the HPR interactions by introducing non-additivity to the contact function.\\

\section{Basic concept of entropic forces}
\label{sec:EntropicForces}

\subsection{Depletion interaction of spherical colloids}

Depletion describes the effect of small solvent particles, like polymers or small hard spheres, on the self-assembly of larger colloids. Already in the 1950s Asakura and Oosawa \cite{AO1954,AO1958} predicted an effective attraction between two plates and between two hard-core spheres within a diluted system of smaller polymers, which was later also revisited by Vrij \cite{V1976}. Moreover, they were able to relate this attractive force to a purely entropically driven effect similar to the entropic self-assembly of colloids into liquid crystal phases. In their calculations, the polymer depletants are modelled as an ideal gas of spheres, which, however, interact via a hard-core potential with the larger colloids. This model of the solvent is also referred to as the penetrable hard spheres model \cite{WR1970,LT2011}. Applying these approximations, the main physical process behind depletion can be simplified.\\

\begin{figure}[t!]
\vspace{-0.6cm}
\centering
\input{chapter_Depletion/depletion_sketch}
\vspace{-0.2cm}
 \caption{The concept of depletion is sketched by the example of two hard-core spherical colloids (left), three hard-core spherical colloids (centre) and two hard-core pear-shaped colloids (right) dissolved in a liquid of smaller hard spheres (indicated in light blue). The system is driven mainly by the entropy of the solvent particles and maximises the free energy by minimising the excluded volume of the bigger colloidal particles. The excluded volume cannot be penetrated by the depletant due to the presence of the colloid (indicated by the dashed line). Thus, the larger objects pack together such that their excluded volumes maximally overlap (indicated in orange) and more space is provided for the depletants. Overall this mechanism can be interpreted as an effective, entropically driven attraction between the colloids.}
\label{fig:DepletionSketch}
\end{figure}


 The free energy $F$ of the system is predominantly governed by the degrees of freedom of the polymer particles. If the number of colloids $N_{\text{coll}}$ is much smaller than the number of solvent particles $N_{\text{depl}}$, that is $N_{\text{coll}}{\ll}N_{\text{depl}}$, the total free energy can be approximated purely by the ideal gas free energy of the depletant (see \eq{eq:HelmholtzFreeEnergy}) \cite{AO1954,K_GS2007}
\begin{equation}
\label{eq:FreeEnergyDepletionIdeal}
F_{\text{depl}} = N_{\text{depl}}\ln\left(\frac{N_{\text{depl}}\lambda^3}{V'}\right)-N_{\text{depl}}.
\end{equation}
with the thermal de Broglie wavelength $\lambda{=}\sqrt{\frac{h^2\beta}{2\pi m}}$ of particles with mass $m$. Furthermore, $V'$ is the volume which is available to the ideal gas. As the solvent cannot penetrate the large colloids we can identify $V'{=}V-V_{\text{excl}}$, where $V$ is the volume of the system and $V_{\text{excl}}$ is the volume, from which the excluded to the solvent by the colloids. Inserting this into \eq{eq:FreeEnergyDepletionIdeal} we get
\begin{equation}
\label{eq:FreeEnergyDepletion}
\begin{aligned}
F_{\text{depl}} &= N_{\text{depl}}\ln\left(\frac{N_{\text{depl}}\lambda^3}{V-V_{\text{excl}}}\right)-N_{\text{depl}}\\ 
&= N_{\text{depl}}\cdot\left[\ln\left(\frac{N_{\text{depl}}\lambda^3}{V}\right)-1\right] + \frac{N_{\text{depl}}}{V}V_{\text{excl}} + \mathcal{O}\left(\frac{V_{\text{excl}}^2}{V^2}\right).
\end{aligned}
\end{equation}

To find the minimum of the global free energy, which is associated with its equilibrium, the system practically minimises $F_{\text{depl}}$ as the contribution of the large colloids and, hence, their degrees of freedom can be neglected. The dominance of the solvent particles implies that the particle configuration tries to decrease $V_{\text{excl}}$ as much as possible, which corresponds to maximising the available space for the solvent spheres. The excluded volume of a single sphere is composed of its volume plus the volume of a thin film or ``envelope'' around the particle with thickness $r_{\text{depl}}$ (radius of depletants) as depicted in \fig{fig:DepletionSketch}. When additional colloids are introduced, their collective excluded volume depends on the position of the colloidal particles. If the colloidal spheres are separated from each other by a distance greater than the solvent diameter the excluded volume is merely a multiple of the excluded volumes of the single spheres. However, if the colloids are within each other's vicinities, such that no solvent particle can be placed between them, the individual excluded volumes overlap and decrease the overall excluded volume. Hence, the entropy maximisation leads to the large colloids coming together as close as possible and form tight clusters (see \fig{fig:DepletionSketch}).\\ 

This behaviour can be interpreted as an effective short-range attraction in addition to the hard-core potential also known as the Asakura-Oosawa potential \cite{AO1954,LT2011}. Note that the attraction results from a purely repulsive system and can then be categorised as an entropic force. The strength of the entropic force can be related to the osmotic pressure which is acting on the colloidal cluster by the depletant. Later the Asakura-Oosawa potential has been improved significantly by extending the theory to finite densities \cite{MCL1995,GED1998} and confirmed using computational simulations \cite{BBF1996,DAS1997}. In this improvements also an entropically driven repulsion was determined for high solvent packing fractions \cite{CNW1996,BBF1996,DAS1997,GED1998}. In this regime, the solvent particles form shells around the colloid leading to effective repulsive forces. The higher order shells around the colloids even cause the depletion forces to oscillate \cite{CMDY1999,RED2000,LALR2002}.\\

 Even though the initial depletion model by Asakura and Oosawa appears to reduce the problem to a very simplified system, the same entropic concept could be applied to other depletion theories which cover more realistic depletant models. Other theories approach polymers for example based on the ideal chain-model \cite{EHD1996,ATL2002}, as hard-core spheres \cite{MCL1995,DAS1997,RED2000}, as hard rods \cite{MCL1997,R2002,LYM2008} or as hard disks \cite{PW2000,HD2004}. Note here, that depletion has been also predicted in classical density functional theory \cite{RED2000,YW2002,OH-GBR2009} (for more information about density functional theory see also \chap{sec:DFT}).\\ 

The first successful attempt to measure depletion forces was made by Evans and Needham, who measured the strength of the attraction between two bilayer membranes in a solution of macromolecules \cite{EN1988}. Later also the second part of the Asakura-Oosawa theory was confirmed experimentally by directly determining the attractive forces between two large hard spheres \cite{CMDY1999}. However, already prior to the direct measurements, many phenomena in systems of hard spherical colloids have been successfully explained by depletion. For example, the ordering of spheres in a solution of polymers close to a hard wall could be attributed to depletion \cite{KFL1994,DWPY1997,KBCS2007}. Also, the demixing of binary hard sphere mixtures into an ordered crystalline cluster of large spheres and a fluid of the small spherical solvent is a result of the excluded volume effects \cite{BH1991,LS1993,R1994,R1995,ID1995,DvRE1999,TRDeK2003}.\\

\subsection{The effect of colloid shape on depletion}

\begin{figure}[b!]
\centering
\input{chapter_Depletion/lock_key_sketch}
\caption{(a) The lock-and-key mechanism in colloidal systems is sketched for hard spheres with concavities within a hard sphere solvent (indicated in light blue). The depletion forces try to minimise the excluded volume (indicated by the dashed line) of the lock (colloids with concavities) and key (colloids without concavities) particles. Hence, depletion leads to the key objects anchoring at the fitting dimples of the lock particles. (b) The time sequence of an experimental system of spherical colloids with and without dimples. The green and red arrows indicate a successful and unsuccessful lock-key binding via depletion, respectively. Scale bar: 2\,$\mu$m. (b) is adapted with permission from \cite{SICP2010}.}
\label{fig:LockKeySketch}
\end{figure}


Similar to other self-assembly processes, the shape of the molecules/colloids naturally impacts how a pair of two colloidal particles in a solvent eventually arranges under the influence of depletion. By changing colloids from a simple sphere to objects with more complicated shapes, the excluded volume does not only depend on the separation but also the relative orientation of the particles (see \fig{fig:DepletionSketch}). Consequently, depletion does not only induce convergence between colloids but also an orientational rearrangement of the particles. For instance, it has been shown that by adding dimples to one of the spheres the other colloid attaches at this concavity \cite{SICP2010,WWZYSPW2014}. This ``lock-and-key'' mechanism can be used as a tool to control the depletion of particles (see \fig{fig:LockKeySketch}). Another sort of directionality can be introduced by creating elongated colloids. At a wall, hard prolate ellipsoids \cite{EBM2003,LM2003_2} and spherocylinders \cite{RvRAMD2002} align with their long axis along the flat interface due to depletion. Moreover, it is known theoretically \cite{ADKF1998,KVKvDPL1999} and from experiments \cite{SYI1989,AF1998} that rod-like colloids self-assemble into clusters with nematic order when non-absorbing polymers are added. Excluded volume mechanisms provide access to rich phase behaviours for various mixtures of hard aspherical particles and depletant particles \cite{ADKF1998,BF2000,DPGAF2004,BDvR2012,AMV2016,GOT2018,GTMOWL2018}, including fascinating effects like depletion induced shape-selective separation in colloidal mixtures by the addition of non-adsorbing polymers \cite{C1942,M2002,BFvHGFLYYCM2010,PKV2010}.\\

Depletion also takes a fundamental role in more complex biological or technological settings, like providing beneficial conditions for polymer crystallisation \cite{KZ2001,TA2002} or describing the physics within the cytoplasm of cells. In the dense and crowded environments of cells \cite{ZT1991,EM2003,RFH2004} the molecular conformations of proteins and other macromolecules are not only influenced by steric interactions but also partially driven by the excluded volume of the molecule \cite{E2001,MFC2006,CG2014}. In biology those effects are mostly known as ``crowding'' \cite{ZM1993,H1996_2,E2001,KTU2014,RM2016}. Prime examples are the influence of crowding agents on protein folding \cite{KTU2014,vdBED1999,E2006}, the stabilisation of helicoidal structures due to excluded volume arguments \cite{MMTB2000,SK2005} or the bundling of fibres or microtubes by introducing polymers \cite{HT2004,HWCHGD2015}. The depletion interactions are known to affect biochemical reactions \cite{M2001,ZRM2008,OCJK2018} and dynamical properties \cite{WZ2008,CKC2012,DHN2014} within cell systems due to its impact on the molecular configurations. It is even argued that the interactions caused by crowding are strong enough to alter observations between in vivo and in vitro experiments, where for the latter the crowded environments tend to be neglected often \cite{RJrCCG1998,M2006,TBF-KHSKLCGPEGS2014,RM2016}.\\

\section{Excluded volume of two pear shaped particles}
\label{sec:ExclVolCalc}

Here we perform numerical calculations to predict the ideal particle arrangement of two pear-shaped particles. For rotationally symmetric particles like pears defined by B\'ezier-curves, three degrees of freedom have to be considered in addition to the particle separation to define a specific constellation between two pears. Two of them can be dedicated to the relative orientations of the particles $\mathbf{u}$ and $\mathbf{v}$. The last one relates to the flexibility to select the contact point $p_c$ on the surface of one colloid, in the case both particles are in touch and the separation is 0. The choices of $\mathbf{u}$, $\mathbf{v}$ and $p_c$, automatically determine the contact point on the surface of the other object. Theoretically, we are able to sweep the whole configurational space of the two-pear-depletion-problem and identify the configuration with the largest excluded volume overlap. The most important steps of the used sampling algorithm are both sketched in \fig{fig:ExclVolAlg} and itemised below:

 \begin{figure}[t!]
\centering
\input{chapter_Depletion/ExclVolAlg}
\caption{The main steps of the algorithm to predict the ideal two pear-shaped particle arrangement in terms of excluded volume. In the first and second step (left) a configuration is chosen, and the surface meshes $B_1$ and $B_2$ of the pear-shaped particles are created. In the third step (centre) the individual excluded volumes of the pears $B'_1$ and $B'_2$ are created by constructing the parallel surface of $B_1$ and $B_2$. Afterwards, (right) the two meshes are merged and the total excluded volume $V_{\text{excl}}$ is computed. The steps are repeated until enough configurations are sampled.}
\label{fig:ExclVolAlg}
\end{figure}
\begin{enumerate}
\item In the first step, an initial arrangement of two pear-shaped particles is chosen. We only consider arrangements where the two pears are in contact, as those configurations provide the minimal excluded volume for convex particles in terms of separation. 
\item Afterwards, the surfaces of the particles are triangulated ($B_1$ and $B_2$). The same method is used for creating the meshes for the HPR model (see \sect{sec:HPR}). 
\item In the next step, the parallel surfaces of the triangulations are generated. The construction of the parallel surface was already introduced in \sect{sec:PearMechanism} (more specifically \eq{eq:ParallelSurfaceMap}), where the vertices of the triangulation are translated in normal direction by $r_{\text{depl}}$. The resulting new meshes $B'_1(r_{\text{depl}})$ and $B'_2(r_{\text{depl}})$ correspond to the interface separating the impenetrable and available space of virtual hard spheres with radius $r_{\text{depl}}$ caused by the first and second pear, respectively. 
\item Subsequently, $B'_1(r_{\text{depl}})$ and $B'_2(r_{\text{depl}})$ are merged to calculate the collective excluded volume defined by $V_{\text{excl}}(r_{\text{depl}}) = B'_1(r_{\text{depl}})\cup B'_2(r_{\text{depl}})$.
\item Another configuration, which has not been observed yet, is chosen and the algorithm returns to step 2. This procedure is repeated until the configuration space is sampled sufficiently densely.
\end{enumerate}

In the following this algorithm is applied to pears with aspect ratio $k{=}3$ and tapering parameter $k_{\theta}{=}3.8$, which, as we showed earlier, lie well within the gyroid phase for the PHGO model (see \fig{fig:PhaseDiagram}) but does not form cubic phases for the HPR-model as indicated in \fig{fig:phase_diagramHard}. Moreover, we use $r_{\text{depl}}{=}0.31\sigma_w$, which corresponds to spheres with $V_{\text{sph}}{=}0.08{\cdot}V_{\text{pear}}$. The computations are performed with the 3D animation software tool Houdini \cite{Houdini}.\\


\begin{figure}[t]
\centering
\vspace{-0.5cm}
\input{chapter_Depletion/ExclVolSph}
\caption{The excluded volume of two pear-shaped particles with $k{=}3$, $k_{\theta}{=}3.8$ and $r_{\text{depl}}{=}0.31\sigma_w$ in relation to the relative orientation of the pears on the unit sphere. The contact point $p_c$ is fixed for the reference pear and chosen such that the configuration with the global minimum can be adopted. In the centre (c), the orientation of the free pear $\mathbf{v}$ is given in spherical coordinates dependent on the orientation of the reference pear $\mathbf{u}$ and the direction towards $p_c$ $\mathbf{u}^{\perp}_1$. On the right, the unit sphere is viewed from the top (d), bottom (e) and side (f) perspective. On the left (a)+(b) two exemplary configurations are shown. The locations of their corresponding orientations $\mathbf{v}_1$ and $\mathbf{v}_2$ on the unit sphere are indicated.}
\label{fig:ExclVolSphere}
\end{figure}

We first show that the three-dimensional excluded volume problem can be narrowed down to its two-dimensional counterpart to sample the configuration space as efficiently as possible. In more mathematical terms, we only consider arrangements of pears where the orientation vectors of the two pears $\mathbf{u}$ and $\mathbf{v}$ and their relative position vector $\mathbf{R}$ are linearly dependent. Only those positions are in line to find the ideal placement of pears. It is somewhat intuitive that, due to the pear's rotational symmetry, the configuration which occupies the least amount of space falls into the category of those linearly dependent arrangements rather than of asymmetric configurations. Moreover, any expansions of the excluded volume in the form of dilatations into the third dimension (like those indicated in \fig{fig:ExclVolAlg}) can be prevented by restricting the particles to a plane. This guess is confirmed by computing the excluded volume for different relative orientations with a fixed contact point $p_c$ of one of the pears as plotted in \fig{fig:ExclVolSphere}c. Here the pear with constant $p_c$ acts as a reference (see \fig{fig:ExclVolSphere}a+b) such that $\mathbf{v}$ can be written in spherical coordinates with respect to the frame defined by $\mathbf{u}$ and $p_c$. The azimuthal angle $\phi{=}0$ of the spherical coordinate system is defined by the direction from the contact point $p_c$ to the centre of the reference pear. For all the tested values of $p_c$, the extremal values in $V_{\text{excl}}$, and hence both its global maximum and minimum, are attained by linearly dependent configurations, that is where the polar angle of $\mathbf{v}$ is either $\phi{=}0$ or $\phi{=}\pi$.\\

To reduce the configuration domain even further, we can utilise another argument about the symmetry of the system. Specifically, the contact, which leads to the maximal or minimal excluded volume, has to be at the same point on both pear surfaces as the choice of the reference pear is arbitrary. Otherwise, the system would have two solutions with the same relative orientations, which is not possible for convex particles. Overall this leaves us with a sampling domain which practically only depends on one degree of freedom, namely on the shared $p_c$. By adding the constraint of linearly dependent orientations with $\phi{=}0$/$\phi{=}\pi$ the polar angle, $\theta$ is restricted to maximally two possible orientations. The excluded volume calculations for the ``roll'' and ``slide'' sampling of the different contact points $p_c$ are plotted in \fig{fig:excluded_V}. 
\begin{itemize}
\item \textbf{Roll route}: The particles start from an antiparallel configuration, when the pears touch with their blunt ends, pass through a parallel alignment next to each other and eventually end up antiparallel again where their pointy ends meet. This sampling can be interpreted as one pear is rolled over the other. 
\item \textbf{Slide route}: During the "slide" sampling the pears are perfectly antiparallel for all $p_c$ which resembles a slide of one pear along the surface of the other. 
\end{itemize}
Hence, the duality of $\theta$ is covered by those two computational pathways. The contact $p_c$ is given by the angle $\beta$ between $\mathbf{u}$ and the normal vector into the pear at $p_c$.\\

\begin{figure}[t!]
\centering
\input{chapter_Depletion/excluded_V}
\caption{The excluded volume of two pear-shaped particles with $k{=}3$, $k_{\theta}{=}3.8$ and $r_{\text{depl}}{=}0.31\sigma_w$ along the ``roll'' (blue) and ``slide'' (red) route, where the particles share the same contact point $p_c$, in terms of the angle $\beta$ between the orientation of the pears and the normal direction into the pear at $p_c$. Both sampling pathways are sketched above. The plots show a minimum of the same value which can be identified as the global minimum of the system. The corresponding optimal configurations are highlighted in the small coloured boxes.}
\label{fig:excluded_V}
\end{figure}

Interestingly, the different paths reveal two distinguishable relative positions at the same contact point $p_c{=}\tilde{p}_c$, which both can be associated with the global minimum of the excluded volume $V_{\text{excl}}$. In one solution the pears are placed side-by-side and oriented perfectly antiparallel towards one another: $\mathbf{u}\cdot\mathbf{v}=-1$ (see \fig{fig:excluded_V}). The minimum, however, does not occur for $\beta{=}\frac{\pi}{2}$ when the pears are at the same height. The particles are rather shifted towards their blunt ends by a small distance. The second ideal configuration exists due to the broken inversion symmetry of the pear-shape and is found when the two pears point roughly in the same general direction (see \fig{fig:excluded_V}). However, here the colloids are not perfectly aligned but slightly tilted towards each other. This tilt also becomes apparent by looking at the excluded volume plot of different orientations at  $\tilde{p}_c$ in \fig{fig:ExclVolSphere}d--f. The top, bottom and especially side view of the unit-sphere clearly show that the minimum at the northern hemisphere is shifted away from the north pole. The tilt can be related directly to the pear-shape. In particular, the angle between the pear-shaped solids is identified as their tapering angle of $\theta_k=15^{\circ}$. Hence, $\theta_k$ also defines the shift in the antiparallel domain, as both optimal configurations are attained for $\tilde{p}_c$.\\

Furthermore, the computations show that configurations, where the blunt ends touch ($\beta{<}\frac{\pi}{2}$ in \fig{fig:excluded_V}), tend to be often more favourable than arrangements where the pears come together with their pointy ends ($\beta{>}\frac{\pi}{2}$). Also in \fig{fig:ExclVolSphere}c a similar observation can be made. If the particle is oriented away from the reference pear and comes in contact with the blunt end, the excluded volume is smaller than if the pear points directly towards $\tilde{p}_c$. This general behaviour indicates that during the rearrangement of inversion asymmetric particles from a separated state due to depletion interactions the colloids are likely to first approach each other with their bigger ends before eventually equilibrating into the most compact formation. This effective blunt end attraction suggests that even the hard HPR pears should have a tendency to cluster with their blunt ends. However, for HPR particles the mechanism seems to be weaker than the tendency in the PHGO model, and not strong enough to lead to equilibrated blunt-end-clustering as we showed in \sect{sec:PhaseDiagramHard}.\\ 

\section[Monte Carlo simulations of depletion effects of pear-shaped particles]{Monte Carlo simulations of depletion effects of pear-shaped particles\sectionmark{MC simulations of depletion effects of pear-shaped particles}}
\sectionmark{MC simulations of depletion effects of pear-shaped particles}
\label{sec:MCDepletion}

Having determined the most favourable conformations of pairs of pear-shaped particles in regards to their excluded volume, we compare the computational predictions to results obtained by computer simulations. Our goal, in particular, to replicate the behaviour of pear-shaped colloids due to depletion and, moreover, to study if the pears indeed prefer the states calculated in \sect{sec:ExclVolCalc}.\\

One very successful theoretical approach to describe depletion is density functional theory (DFT) which is discussed in more detail in \chap{sec:DFT}. Roth introduced a so-called ``insertion approach'' \cite{RED2000,KRD2006} within DFT, where the depletion potential is calculated from the solvent density distribution close to one fixed colloid by insertion of a second colloidal particle and use of the potential distribution theorem \cite{H1983}. The interactions in a mixture of hard spheres \cite{RED2000}, a system of a spherocylinder close to a hard wall \cite{RvRAMD2002}, and a mixture of aspherical, but inversion symmetric particles \cite{KRD2006} have been derived with this ansatz. Also, other theories have been applied to calculate depletion interactions \cite{BBF1996,DAS1997,K2004} but have shown to be less efficient as every single configuration has to be treated individually. However, all those theoretical approaches only cover a set of particles with simple shapes and have not been applied to pear-shaped particles prior to this thesis. This difficulty is enhanced even more as we would have to develop a functional of orientational-dependent contact functions like for PHGO particles. We will derive a density functional for hard pear-shaped particles later in \sect{sec:PearFMT}, such that we might be able to implement a theoretical description of the pear-shaped particle depletion based on DFT in the future.\\

Alternatively, depletion interactions have been obtained with Monte Carlo simulation techniques. A typical procedure to calculate the depletion forces between various particles is the ``acceptance'' approach where the free energies between two different configuration states are compared. During these simulations, the positions and orientations of both colloids are fixed, and only the hard sphere solvent is displaced in the process of the Monte Carlo step. Finally, the free energy difference between two states can be related to the acceptance rate to jump from one colloid particle's relative position to the other and vice versa without causing particles to overlap \cite{B1976,AT1991,LM2002,LM2003_2}. This procedure has been advanced using Wang-Landau Monte Carlo approaches \cite{WL2001,SDP2002,MLM2014,HKHS2016}. Also, a hybrid of simulation and DFT has been suggested \cite{JW2011}. Those approaches are, however, very complicated for the pear shape (in case of the hybrid approach) or very time inefficient, as for every configuration state a separate MC run has to be performed in the acceptance approach. Combining these issues with the already computationally demanding overlap check between two meshes for the HPR particles and hard spheres (see \sect{sec:PotentialHard}), the mentioned techniques are all impracticable. However, in general, we are not necessarily interested in the specific free energy-calculations of the different states but merely want to clarify the distinctions between the HPR and PHGO model. Therefore, the question of depletion is tackled by applying Monte-Carlo simulations in the following and more straightforward fashion.\\

\subsection{Depletion interactions between HPR particles}

Monte Carlo simulations are performed on systems with $N_{\text{pear}}{=}2$ hard-core pear-shaped particles within a solvent, which is approximated by a large number $N_{\text{sph}}{=}1498$ of surrounding smaller hard spheres, within a cubic box with periodic boundary conditions in all three dimensions. The aspect ratio $k{=}3$ and tapering parameter $k_{\theta}{=}3.8$ of the pear-shaped particles are chosen to easily compare the simulation results with the calculations of \fig{fig:ExclVolSphere}. For the same reason the sphere radii of the solvent $r_{\text{depl}}$ is set to $0.31\sigma_w$, which corresponds to the volume ratio between the spheres and pears $v{=}\frac{V_{\text{depl}}}{V_{\text{pear}}}=0.08$. An acceptance rate of roughly 50\,\% has been achieved by setting the maximal translation $\Delta_{q,\text{max}} {=} 0.085\sigma_w$ and the maximal orientational displacement $\Delta_{u,\text{max}}{=}0.085\sigma_w$ per step.  The greater number of depletants assures that the simulations are not affected by the boundary conditions and the system can indeed be interpreted as two pear colloids within a sea of a hard sphere solvent. Furthermore, the sphere size is small enough to see depletion interactions between the particles occurring at higher densities. All sets are performed in the $NVT$-ensemble starting from different diluted initial states at 
\begin{equation}
\label{eq:GlobalDensityMixture}
\rho_g=\frac{N_{\text{pear}}{\cdot}V_{\text{pear}}+N_{\text{sph}}{\cdot}V_{\text{sph}}}{V_{\text{box}}}=0.1.
\end{equation}
After a sequence of compressions to the final density $\rho_g{=}0.45$  the system is studied for $5.0{\cdot}10^{6}$ steps.\\

\begin{figure}[t!]
\centering
\input{chapter_Depletion/separation}
\caption{Representative progressions of the separation $R$ of two pear-shaped particles (red: HPR, blue: PHGO, orange: NAHPR.) in a sea of 1498 hard spheres, acting as a solvent during the Monte-Carlo simulations. The simulations are performed at a global density of $\rho_g{=}0.45$. All models show an effective attraction into the zone of influence induced by depletion effects. The shaded area approximates this zone of influence where the particles can be considered in contact.}
\label{fig:SeparationDepletion}
\end{figure}

We first simulate HPR pears in a hard sphere fluid. As we perform MC simulations, we can use the hard sphere-pear interactions based on the sampled B\'ezier-contour as described in \sect{sec:PearShape}. For every simulation run, the entropic depletion attraction between the pear-particles can be noticed when the colloids are in each other's vicinity, which means that their excluded volumes overlap. More precisely, the particles stay together for a considerable number of MC steps (see \fig{fig:SeparationDepletion}), which leads to the conclusion that the system indeed favours the particles coming in contact. However, the entropic attraction seems to be short range and rather weak. This can be seen in \fig{fig:SeparationDepletion}, where the particles often separate again from a nearby configuration after some MC steps before they typically approach their zone of influence again. Here, we have to mention once more that this ``approach'' is not dynamic. Nevertheless, the preferred sampling of close pear arrangements is a strong indication for depletion interactions.\\

\begin{figure}[t!]
\centering
\input{chapter_Depletion/ori_hard}
\caption{The relative orientation (a) and lateral distance distribution (b) of two HPR particles in a sea of 1498 hard spheres, acting as a solvent at global density $\rho_g=0.45$, on the left. The particle parameters are set to $k=3$, $k_{\theta}=3.8$ and $r_{\text{depl}}=0.31\sigma_w$ ($\frac{V_{\text{depl}}}{V_{\text{pear}}}=0.08$). Only pair-configurations are considered if the pear-shaped particles are close to each other such that the excluded volumes overlap. Positive angles $\alpha$ indicate V-configurations (blunt ends together), whereas negative $\alpha$ values describe A-configurations (pointy ends together). On the right, two typical arrangements, extracted from the simulations, are shown. The top snapshot (dashed line, (c)) corresponds to the indicated peak and coincides with the parallel solution for maximal excluded volume overlap. The bottom configuration (dash-dotted line, (d)) contributes to the second peak and matches the anti-parallel solution in terms of minimised excluded volume.}
\label{fig:ori_hard}
\end{figure}

Even though the particles are affected by the presence of the second colloid, the determination of the relative arrangements of the colloid pair faces some difficulties. The main issue which has to be overcome is poor statistics. As we are studying a two-particle problem, it is hardly feasible to gather enough data for a detailed combined analysis of the possible states due to computational time constraints. Therefore, we decouple the degrees of freedom and only investigate one relative parameter at a time. In \fig{fig:ori_hard}a the relative polar angle between two close HPR particles is plotted. For these plots, only configurations are considered if the excluded volumes overlap. This ensures that the sampled relative orientations are actually influenced by the close distance between the particles. The relative angle $\alpha$ between the orientation vectors of the pears $\mathbf{u}$ and $\mathbf{v}$ is split into two domains to characterise the orientational states further. For positive angles, the pears point away from each other such that their blunt ends are in contact. A negative angle indicates that the pears face towards one another and that their pointy ends are closer together. In the following we will refer to these two domains ``V''-configurations ($\alpha{>}0$) and ``A''-configuration ($\alpha{<}0$).\\

The histogram of the relative pear orientations shows three distinct peaks which match perfectly with the ideal configurations predicted in \fig{fig:ExclVolSphere}c and \fig{fig:excluded_V}. The first preferred orientation is measured at $\alpha{=}{-}0.26{=}{-}15^{\circ}$, and hence categorised as an A-configuration. This relative angle corresponds directly to the parallel solution for minimal excluded volume as it coincides with the tapering angle $\theta_k{=}15^{\circ}$. The configuration can also be extracted from the simulations directly (see a snapshot in \fig{fig:ori_hard}c). The second and third peak at $\alpha{=}\pm\pi{=}\pm 180^{\circ}$ can be combined into a single characteristic orientation due to the duality of the A- and V-configuration for $\cos(\alpha){=}-1$. Moreover, this orientation also coincides with the predictions as it fits the second solution of the excluded volume calculations, where the particles are aligned anti-parallelly next to each other. A snapshot from the MC simulation of this particular configuration is depicted in \fig{fig:ori_hard}d.\\ 

The observations are corroborated by the lateral distance distribution between two particles when in contact. \fig{fig:ori_hard}b highlights that the neighbouring pears are not distributed around the centre point of the reference particles. The distribution is rather slightly shifted towards the pointy end. The inversion asymmetric shape of the HPR particle consequently introduces a move of the optimal contact point above the centre-point. Hence, the HPR particles behave precisely as expected according to \sect{sec:ExclVolCalc} and according to the solutions of the ideal configurations to maximise the available space for the hard spheres.\\
   
\subsection{Depletion interactions between PHGO particles}
\label{sec:DepletionPHGO}

We established that the HPR particle model describes the imposed pear-shape very well in terms of depletion and reproduces the analytical predictions. Therefore, it acts perfectly as a reference for other models which describe pear-shaped particles like the PHGO model. This gives us an excellent opportunity to study the ramifications to describe a pear using a hard Gaussian overlap approach. Thus, the depletion MC simulations are repeated. The same parameters are applied except that the HPR contact function is replaced with the PHGO contact function to approximate the particle overlap.\\

The first distinction between the PHGO and HPR system becomes apparent during the MC sampling already. By tracking the distances between both particles for every MC step in \fig{fig:SeparationDepletion} the depletion attraction between two PHGO pears seems to be much stronger than in the equivalent HPR case. This can be explained by the development of the separation once the two PHGO pears are close together. After the pears pass a sequence of arbitrary displacements and eventually approach each other, the touching configuration stays stable.\footnote{During the simulations of the PHGO pears a separation has been observed only once out of fifty runs.} This is in contrast to the occasional split-ups of the HPR particles where more prolonged periods of configurations close together alternate with stages of separation and subsequent recombination. This means the depletion attraction is of the order of $k_BT$ or less for HPR and considerably more for PHGO particles. The increased strength of the entropic force, however, can be related to the contact function of the PHGO pear. Presuming the particles are in the optimal state, an attempted translational step and especially an attempted rotational step is much more strongly penalised for PHGO than for HPR particles. This is manifested in the contact profile of roughly perpendicular arrangements. Here, the pear size is overestimated, and a particle pair is accounted as overlapping even though they are not in contact according to the B\'ezier-curve depiction (see \fig{fig:PearContactFunc} for a comparison of the contact profiles between PHGO and HPR model). The effect is comparable to the PHGO pears and HGO ellipsoids \cite{P2008} entering orientationally ordered phases already for low densities. The depth of the effective potential does not necessarily indicate that the two models differ qualitatively, but suggests that the depletion is more guided towards the equilibrium states.\\

\begin{figure}[t!]
\centering
\input{chapter_Depletion/ori_go}
\caption{The relative orientation (a) and lateral distance distribution (b) of two PHGO particles in a sea of 1498 hard spheres, acting as a solvent at global density $\rho_g=0.45$, on the left. The particle parameters are set to $k=3$, $k_{\theta}=3.8$ and $r_{\text{depl}}=0.31\sigma_w$ ($\frac{V_{\text{depl}}}{V_{\text{pear}}}=0.08$). Only pair-configurations are considered if the pear-shaped particles are close to each other and the excluded volumes overlap. Positive angles $\alpha$ indicate V-configurations (blunt ends together). Negative $\alpha$ values describe A-configurations (pointy ends together). This is also indicated above the plot. On the right two typical arrangements, extracted from the simulations, are shown. The top snapshot (dotted line, (c)) shows a V-configuration, which corresponds to the indicated peak. This configuration does not coincide with the parallel solution for maximal excluded volume overlap of B\'ezier pears. The bottom configuration (dash-dotted line, (d)) contributes to the second peak and matches the anti-parallel solution in terms of minimised excluded volume.}
\label{fig:ori_go}
\end{figure}

The relative orientation distribution between two PHGO particles in close contact is plotted in \fig{fig:ori_go}a. Two distinct peaks are perceivable similar to the equivalent HPR system. The main peak is found at $\alpha{=}\pm\pi$ which again corresponds to an antiparallel configuration. Therefore, the orientation distribution suggests that the PHGO pear model reproduces the antiparallel solution sufficiently. In this domain, the HPR and PHGO differ the least from each other, such that it is quite intuitive that in the antiparallel case both models share the same solution. Additionally, we can find many configurations as depicted in \fig{fig:ori_go}d, which contribute to the pronounced peak at $\alpha{=}\pm\pi$ and coincide with the ideal solution to a sufficient degree. By focusing on the second minor peak, however, we observe two major differences compared to the HPR system. Firstly the peak is significantly less intense. This indicates that for PHGO particles the antiparallel configuration is more beneficial than the parallel solution. This is again explained by the equivalence of the HPR and PHGO contact profile for antiparallelly aligned particles. By changing the relative angle between the pear-shaped particles, the overlap tends to be overestimated by the PHGO model which consequently leads to a higher excluded volume. Thus, the duality of the ideal configuration is broken by the particular angle dependence of the PHGO contact function and weighted to the benefit of antiparallel arrangements.\\

 The second difference is the position of the peak, which is shifted from $\alpha{=}-15^{\circ}$ to a positive value close to $\alpha{=}20^{\circ}$. Hence, the particles form V-configurations rather than the expected A-configurations. To clarify the reason behind this transition we take a closer look at those V-configurations which can be obtained from the simulations directly. A representative pair is portrayed in \fig{fig:ori_go}c. It becomes apparent that the pears slightly overlap. Here, the term ``overlap'' might be misleading as the particles do not technically overlap in terms of their PHGO contact function but according to the best possible illustration using the B\'ezier representation. However, it also has to be mentioned that the spheres interact with the pear according to this B\'ezier shape. Thus, the solvent particles effectively experience the pear shape differently than another PHGO particle. Furthermore, the underlying underestimation of the PHGO-contact function enables the pear-shaped particles to occupy space, which by design cannot be reached by hard spheres and would also be prohibited for HPR particles. This effect is known as \textit{non-additivity} and is well studied for hard binary sphere mixtures \cite{BPGG1986,LALA1996,RE2001,HS2010,ZFLSSO'H2015}, which successfully model the behaviour of binary alloys \cite{KA1995,SKCFC2011} or organic mixtures \cite{M1977,PM2006}. It is known that non-additivity leads to repelling and attracting effects \cite{RE2001,W-CH2011}, which open the door for exotic crystalline phases \cite{PM2006,W2010} and also shift the critical demixing density to lower values \cite{D1998,LFH2000}. Already Asakura and Oosawa studied a non-additive system to describe the depletion interactions where the large colloids ``see'' the polymers as hard spheres with finite radius whereas the polymers act as point particles among themselves \cite{AO1954}.\\
 
The V-configurations can also be associated with non-additivity effects between two PHGO pears. Here the excluded volume is decreased instead of simple alignment by an alternative route, namely by increasing the overlap of the two particles due to non-additivity. For pears with $k{=}3$ and $k_{\theta}{=}3.8$ the maximal overlap occurs roughly at an angle of $\alpha_{\text{overlap}}{\approx}30^{\circ}$. This is considerably higher than the measured angle between the pears in the V-configuration observed in the simulations. However, we can argue that the adopted angle results from the intricate interplay of reducing excluded volume via overlap and alignment and the sphere radius of the solvent. For small volume ratios the overlap is more dominant and the V-arrangement more favourable, whereas for large ratios the contribution of the overlap becomes negligible and the aligned A-configuration will be adopted.\\
 
 To complete the comparison between the HPR and PHGO particles, we investigate the lateral distance of the PHGO pears to its fellow pear in close contact in \fig{fig:ori_go}b. Compared to \fig{fig:ori_hard}b the distribution is much narrower which leads the impression that the HPR particles are more flexible to obtain the equilibrium state whereas the PHGO pears are more restricted in terms of fluctuations from the ideal configuration. The emergence of the narrow peaks can again be attributed to the non-additive characteristics of the PHGO model. Furthermore, the two maxima indicate the existence of two different contact points. One is associated with the V position ($z<0$), the other peak can be identified as the contact for the antiparallel solution $z{>}0$.\\

\section{Conclusion and outlook}
\label{sec:OutlookDepletion}

In this chapter, we studied depletion effects on pear-shaped particles due to a solvent of hard spheres as preparation for \chap{sec:Mixtures} where the range of mixture is expanded. To this end, we investigated the depletion interactions of a pair of pear-shaped particles in a sea of a hard sphere solvent. In the course of this study, we first determined the optimal pear configurations in terms of minimised total excluded volume based on the B\'ezier curves to predict the equilibrated particle formation. Using numerical calculation techniques, we could compute two global minima; a parallel and antiparallel solution, which both share the same contact point on the pear surface. Both configurations could be related directly to the taper of the particle. Afterwards, the predicted states could be obtained in Monte Carlo simulations of two HPR pear particles dissolved in a hard sphere solvent. However, depletion attraction is weak for the chosen parameters.\\ 

In comparison, the PHGO pear particles revealed differences to the predictions. Even though the antiparallel configuration was also reproduced for PHGO pears, the parallel solution was found to be less dominant and shifted from an A- to a V-configuration with a different contact point. We argued that the V-configuration is governed by the PHGO contact function which underestimates the pear overlap slightly and causes overlaps. Moreover, it has been shown that the depletion attraction between two PHGO particles is much stronger than between HPR particles.\\

\begin{figure}[t!]
\centering
\vspace{-0.2cm}
\input{chapter_Depletion/shape_nonadd_docking}
\caption{The procedure to obtain the second mesh in the NAHPR model which determined the overlap between the blunt ends of two pears with $k=3$ and $k_{\theta}=3.8$. First, two pears are placed symmetrically at an angle $\alpha=30^{\circ}$ such that the pears are exactly in contact according to the PHGO contact function. The distance is decreased by $-0.035\sigma_w$ also to compensate the contact overestimation for A-configurations.  Afterwards, the overlap is cut from the initial contour (dashed) such that a concavity occurs (dotted line). The equivalent non-additive contour is obtained from its convex hull (dash-dotted). This procedure is repeated for different angles between $\alpha=30^{\circ}\pm15^{\circ}$. The final contour (solid line) is the basis of the solid of revolution from which the mesh is generated.}
\label{fig:HPRmodified}
\end{figure}

The discrepancies in the depletion behaviour also give improved insight into the diminished and aided spontaneous creation of bilayer-phases in monodisperse HPR and PHGO particle systems, respectively. It is more than likely that specific details of the relative positions between neighbouring pear-shaped particles are varied due to the enhanced complexity of the excluded volume effects in one-component assemblies. Nevertheless, we can reason that the quality of the arrangements would not change and hence, general statements about the local formations can be made. Especially three contributions to the stabilisation mechanisms of bilayer configurations are identified.
\begin{enumerate}
\item By breaking the duality of the optimal configurations the systems introduce a local polar order. In the PHGO model, this leads to a dominant formation of antiparallel alignments between adjacent pears. This exact orientational order is also observed in the pair-correlation functions weighted with the polar order parameter of the one-component PHGO-particle systems (see \fig{fig:PairCorHard} in \sect{sec:PhaseDiagramHard}). Hence, the system is guided towards the formation of ``zig-zag''-patterns, which are a prerequisite of interdigitated bilayers.
\item The interdigitation is enhanced by the preferred parallel order into V- rather than A-configurations. It is quite intuitive to imagine that sheets, which consist of an array of V-aligned pears, interlock analogous to a zip mechanism and subsequently develop bilayers.
\item The greater fluctuations of the contact point in HPR systems hinder a targeted alignment of particles. This consequently leads to an increased susceptibility for defects within the bilayers, and a weaker correlation of translational order as those observed in typical smectics let alone gyroid or lamellar phases. 
\end{enumerate}
These three factors raise the question of how pear-shaped particles adopting bilayer phases can be realised in experiments. Assuming that colloids interacting via the HPR potential will be more likely to be synthesised in the future\footnote{This assumption is merely based on the fact that the HPR contact profile resembles the B\'ezier shaped more closely than the PHGO model. However, if this premise is indeed true cannot be answered to date as modern-day synthesis techniques do not yet offer the amount of detail that is needed.}, the question can be rephrased as such. How does the HPR contact profile have to be modified to obtain the key characteristics of the PHGO contact function? In the following, we want to propose a promising approach as an outlook and introduce non-additive features to the mesh-description of pears as well.\\

\begin{figure}[t!]
\centering
\vspace{-0.5cm}
\input{chapter_Depletion/nonadd}
\caption{The concept of the overlap determination for the NAHPR model. The pear consists of an inner contour (solid line, non-additive part) and an outer contour (dotted line, similar to the HPR model). If the pears coms together with their blunt ends (left) the particles are considered in contact if their inner contours touch. Otherwise (centre) the outer contours determine the overlap. The interactions with hard spheres are also according to the outer contour (right).}
\label{fig:nonaddArangement}
\end{figure}

The non-additive features are added to the blunt ends of the pear particles. Using this approach we specifically try to engineer an HPR potential which favours the formation of V-configurations due to depletion interactions. The mesh which describes the interaction between two blunt ends is based on the distance of two PHGO particles with the largest overlap. As already mentioned this occurs for $\alpha_{\text{overlap}}{=}30^{\circ}$. However, the distance is decreased even a bit further by $-0.035\sigma_w$ to additionally compensate for the contact overestimation for A-configurations which otherwise would not be considered. The contour of the non-additive shape is created by introducing a flat line between the two points where both B\'ezier curves meet (see \fig{fig:HPRmodified}). Taking this new contour as a basis, we repeat the procedure for different angles $\alpha{=}30^{\circ}{\pm}10^{\circ}$ to allow some flexibility of the adopted orientations. Afterwards, a triangulated mesh of the solid of revolution of the resulting contour is generated. The mesh is implemented into the MC algorithm such that only the blunt ends of the pears are allowed to overlap according to the B\'ezier shape. To put it differently, the particles interact via the non-additive mesh exclusively if the particles come together with their blunt ends. Otherwise, the overlap is determined by the regular mesh describing the pear surface (see \fig{fig:nonaddArangement}). Furthermore, the pear-sphere interactions stay unmodified such that the hard solvent still experiences the HPR pear. We will refer to this model as the non-additive hard pears of revolution (NAHPR) model. In experiments, the underlying contact function might be realised by preparing pear colloids with a rougher surface at the pointy than at the blunt ends. By using different roughness, the strength between different parts of a colloid can be controlled, and therefore an effective entropic attraction between specific moieties of the colloid can be introduced \cite{ZM2007,KNSHYWvBGDK2012}.\\

\begin{figure}[t!]
\centering
\vspace{-0.7cm}
\input{chapter_Depletion/ori_nonadd}
\caption{The relative orientation (a) and lateral distance distribution (b) of two non-additive HPR particles in a sea of 1498 hard spheres, acting as a solvent at global density $\rho_g=0.45$, on the left. The particle parameter are set to $k=3$, $k_{\theta}=3.8$ and $r_{\text{depl}}=0.31\sigma_w$ ($\frac{V_{\text{depl}}}{V_{\text{pear}}}=0.08$). Only pair-configurations are considered if the pear-shaped particles are close to each other and the excluded volumes overlap. Positive angles $\alpha$ indicate V-configurations (blunt ends together). Negative $\alpha$ values describe A-configurations (pointy ends together). This is also indicated above the plot. On the right two typical arrangements, extracted from the simulations, are shown. The top snapshot (dotted line, (c)) corresponds to the indicated peak and shows the engineered V-configuration. The bottom configuration (dash-dotted line, (d)) is a defect of the non-additive mesh and contributes next to the anti-parallel solution also to the second indicated peak.}
\vspace{-0.3cm}
\label{fig:ori_nonadd}
\end{figure}

After implementing the non-additive contact function, the depletion MC simulations are again repeated with the same parameters. Both \fig{fig:SeparationDepletion} and \fig{fig:ori_nonadd} reveal that some of the features of the PHGO model have been adopted by the NAHPR model. By investigating the separation during the MC simulation in \fig{fig:SeparationDepletion} it becomes apparent that the depletion interaction increases. Even though the PHGO particles still show stronger attraction, the NAHPR particles remain in the zone of influence similarly as soon as they are within their vicinities. More interesting, however, is the orientation distribution for NAHPR particles in contact (see \fig{fig:ori_nonadd}a). The non-additivity at the blunt ends indeed stabilises the desired V-configurations creating a dominant peak at around $\alpha{=}20^{\circ}$. Nevertheless, by taking a close look, a small peak at the A-configurations can be observed as well. This leads to the conclusion that two minima for the excluded volume can be obtained within the parallel configurations. The global one is attributed to the V-configuration and the non-additivity, the second minor one can be ascribed to the A-position and the parallel alignment of the pears according to their tapering parameter.\\

However, the NAHPR model still does not recreate all feature of the PHGO-particles perfectly. Especially the lateral distance distribution in  \fig{fig:ori_nonadd}b does not reproduce the two narrow, distinct peaks. The distribution is still rather broad, even though most of the contact points are located underneath the centre point of the pear-shaped particle. Moreover, some of the simulations end up in configurations which contribute to the preferred antiparallel alignment but do not coincide with the prediction. Although the prediction is still the dominant configuration, the non-additivity allows the particles also to overlap with the blunt ends in an antiparallel configuration (S-configuration, see  \fig{fig:ori_nonadd}d) and also introduces in the antiparallel case a secondary minimum.\\

To put it in a nutshell, the NAHPR particles can recreate some of the features of the PHGO contact function, like the formation of V-configurations or the enhanced depletion attraction. Some other features like the symmetry breaking into heavily favoured anti-parallel configuration could not be resolved by the modified model yet. However, the introduction of non-additivity between blunt ends seems to be a pivotal factor to enable bilayer formation. The present issues might be resolved by further alternations of the NAHPR interactions. One solution might be to add additional angle dependence to the non-additivity, such that blunt ends are only able to overlap if the particles are pointing roughly in the same direction. This would probably diminish the formation of S-configurations. Another approach might be to replace the rounded pear surface with a partially flat surface. This would allow us to control not only the non-additivity attraction but also the depletion attraction via alignment by introducing more or less curvature to the surfaces.

